A Survey on Multimodal Large Language Models for Autonomous Driving

With the emergence of Large Language Models (LLMs) and Vision Foundation Models (VFMs), multimodal AI systems benefiting from large models have the potential to equally perceive the real world, make decisions, and control tools as humans. In recent months, LLMs have shown widespread attention in autonomous driving and map systems. Despite its immense potential, there is still a lack of a comprehensive understanding of key challenges, opportunities, and future endeavors to apply in LLM driving systems. In this paper, we present a systematic investigation in this field. We first introduce the background of Multimodal Large Language Models (MLLMs), the multimodal models development using LLMs, and the history of autonomous driving. Then, we overview existing MLLM tools for driving, transportation, and map systems together with existing datasets and benchmarks. Moreover, we summarized the works in The 1st WACV Workshop on Large Language and Vision Models for Autonomous Driving (LLVM-AD), which is the first workshop of its kind regarding LLMs in autonomous driving. To further promote the development of this field, we also discuss several important problems regarding using MLLMs in autonomous driving systems that need to be solved by both academia and industry.

==> sec/planning.tex <==
\subsection{Multimodal Language Models for Planning}

Motion or trajectory planning is critical for the safety of autonomous vehicles. The objective of motion planning is to determine the optimal path that avoids collision, minimizes travel costs, and satisfies other constraints, such as the comfort of passengers and conforming to traffic regulations. Herein, planning models act as the decision-makers and require a sufficient understanding of their surroundings to guarantee reasonable outcomes. LLMs are well-known for their power in reasoning with common senses~\cite{zhou_common_2020}. Therefore, we have observed emerging interests in implementing these models for robotic planning in the past few years.

In most existing methods, LLMs serve as the bridge to support human-machine interactions. For general purposes, LLMs can be task-agnostic planners. In~\cite{huang_language_2022}, the authors discovered that pre-trained LLMs contain actionable knowledge for coherent and executable action plans without additional training. Huang et al.~\cite{huang_voxposer_2023} proposed the use of LLMs for converting arbitrary natural language commands or task descriptions into specific and detail-listed objectives and constraints. In the use cases of autonomous vehicles, \cite{wen2023dilu} proposed integrating LLMs as decision decoders to generate action sequences following chain-of-thoughts prompting. In \cite{cui_drive_2023}, authors showcased that LLMs can decompose arbitrary commands from drivers to a set of intermediate phases with a detailed list of descriptions of actions to achieve the objective.

Meanwhile, safety is essential for autonomous driving. The power to comprehend its surroundings and the transparency of the decision process are also important. 

In the field of robotics, previous works showed that LLMs could enable reasoning of planning~\cite{wang_voyager_2023,pmlr-v205-shah23b}, perceiving the environment with textual description~\cite{huang_inner_nodate,zeng_socratic_2022,10161317}, and reward specification in reinforcement learning for extrapolating user preferences. 

For context understanding in autonomous driving,~\cite{kim2018textual} showcased that video-to-text models can help generate textual explanations of the environment aligned with downstream controllers. Deruyttere et al.~\cite{deruyttere_talk2car_2019} demonstrated that LLMs can identify specific objects in the surroundings that are related to the commands or descriptions in natural language. For the explainability of the model, Xu et al. ~\cite{xu_drivegpt4_2023} proposed to integrate LLMs to generate explanations along with the planned actions. In~\cite{cui_receive_2023}, the authors proposed a framework where LLMs can provide descriptions of how they perceive and react to environmental factors, such as weather and traffic conditions.

Recently, the progress in MLLMs greatly improved the potential of LLMs to serve as a general and safe planner model for autonomous driving. The ability to process and fuse visual signals such as images enhanced navigation tasks by combining visual cues and linguistic instructions \cite{kamath_new_2023,ku_room-across-room_2020}. Interoperability challenges have historically been an issue for autonomous planning processes \cite{gohel_explainable_2021,chib_recent_2023}. 
However, recent advancements in addressing interoperability challenges in autonomous planning have leveraged the impressive reasoning capabilities of MLLMs during the planning phases of autonomous driving \cite{fu_drive_2023,cui_drive_2023,chen_driving_2023}. In one notable approach, Fu et al. \cite{chen_driving_2023} integrated vectorized object-level 2D scene representations into a pre-trained LLM with adapters, enabling direct interpretation and comprehensive reasoning about various driving scenarios. Meanwhile, Cui et al. \cite{cui_drive_2023} introduced a framework that utilizes LLMs to provide a step-by-step explanation of the decision-making process. Additionally, Fu et al. \cite{fu_drive_2023} employed LLMs for reasoning and translated this reasoning into actionable driving behaviors, showing the versatility of LLMs in enhancing autonomous driving planning. Additionally, GPT-Driver \cite{mao_gpt-driver_2023-2} reformulated motion planning as a language modeling problem and utilized LLM to describe highly precise trajectory coordinates and also its internal decision-making process in natural language in motion planning. \cite{keysan2023text} investigated the utilization of textual descriptions along with pre-trained language encoders for motion prediction in autonomous driving.

% Motion or trajectory planning is critical for the safety of autonomous vehicles. Planning aims to decide the optimal path that avoids collision, minimizes travel costs, and satisfies other constraints, such as the comfort of passengers and conforming to traffic regulations. Herein, planning models act as the decision-makers to derive the optimal path conditioned on observations of the surroundings. Classic models implement a vision-based pipeline, where they are designed to extract meaningful information from images~\cite{hu_joint_2019, liu_vehicle-related_2020, li_bevformer_2022}, point clouds~\cite{wang_map-based_2017, wang_pedestrian_2017, zhao_detection_2019}, or data collected by other visual sensors~\cite{cui_radar_2023}. CNNs are the most commonly used in these models to process rasterized data like images, while Graph Neural Networks (GNNs) and Transformer architectures are emerging solutions for processing vectorized data like point clouds or HD maps. Nevertheless, these classic vision-based models understand the world only using visual sensors, which ignores the feedback from passengers or drivers.

% With significant progress in LLMs, many recent works highlight their essential roles in human-machine interactions. Specifically, LLMs can be task-agnostic planners~\cite{huang2023voxposer} that convert arbitrary commands or descriptions from human instructors into specific and detail-listed objectives and constraints. Therefore, applications using LLMs for planning in robotics have become an active area for the past few years. The main focus of these existing works lies in the reasoning of planning~\cite{wang_voyager_2023,pmlr-v205-shah23b}, perceiving the environment with textual description~\cite{huang_inner_nodate,zeng_socratic_2022,10161317}, and reward specification in reinforcement learning for learning user preferences. Moreover, recent progress in multi-modal language model~\cite{huang2023chatgpt} demonstrates great potential to incorporate vision data to enhance performance. However, we note that applications of LLMs for autonomous vehicles are underexplored. Extensive research can address aspects including using LLMs as few-shot or zero-shot adapters~\cite{NEURIPS2020_1457c0d6, wei2022finetuned,pmlr-v162-wang22u} for transferring motion planning models across different traffic scenarios, enabling vehicle manipulations considering driver or passenger preferences, and dynamic strategy reasoning guided by chain-of-thoughts prompting.


% MLLMs have significantly influenced the development of autonomous driving technology, with researchers acknowledging their robust reasoning and common-sense abilities \cite{bian_chatgpt_2023-1, chowdhery_palm_2022, ouyang_training_2022, chung_scaling_2022}. The integration of language into planning processes has a rich history, dating back to early work that used language to instruct robots \cite{kress-gazit_translating_2008}. Subsequently, Matuszek et al. explored the parsing of natural language commands into actionable instructions and control structures \cite{desai_learning_2013}. More recently, multi-modal language models have enhanced navigation tasks by combining visual cues and linguistic instructions \cite{kamath_new_2023,ku_room-across-room_2020}. Interoperability challenges have historically been an issue for autonomous planning processes \cite{gohel_explainable_2021,chib_recent_2023}. 
% However, recent advancements in addressing interoperability challenges in autonomous planning have leveraged the impressive reasoning capabilities of MLLMs during the planning phases of autonomous driving \cite{fu_drive_2023,cui_drive_2023,chen_driving_2023}. In one notable approach, Fu et al. \cite{chen_driving_2023} integrated vectorized object-level 2D scene representations into a pre-trained LLM with adapters, enabling direct interpretation and comprehensive reasoning about various driving scenarios. Meanwhile, Cui et al. \cite{cui_drive_2023} introduced a framework that utilizes LLMs to provide a step-by-step explanation of the decision-making process. Additionally, Fu et al. \cite{fu_drive_2023} employed LLMs for reasoning and translated this reasoning into actionable driving behaviors, showing the versatility of LLMs in enhancing autonomous driving planning. Additionally, GPT-Driver \cite{mao_gpt-driver_2023-2} reformulated motion planning as a language modeling problem and utilized LLM to describe highly precise trajectory coordinates and also its internal decision-making process in natural language in motion planning. \cite{keysan2023text} investigated the utilization of textual descriptions along with pre-trained language encoders for motion prediction in autonomous driving.
